Black Hole Binary Dynamics from the Double Copy and Effective Theory

We describe a systematic framework for computing the conservative potential of a compact binary system using modern tools from scattering amplitudes and effective field theory. Our approach combines methods for integration and matching adapted from effective field theory, generalized unitarity, and the double-copy construction, which relates gravity integrands to simpler gauge-theory expressions. With these methods we derive the third post-Minkowskian correction to the conservative two-body Hamiltonian for spinless black holes. We describe in some detail various checks of our integration methods and the resulting Hamiltonian.

==> figs/twoloop_cuts.tex <==
% !TeX root = ./overall_paper.tex
%\section{Integrands at Two Loops Using Four-Dimensional Helicity}
%\label{TwoLoopSection}

%%%%%%%%%%%%%% FIGURE %%%%%%%%%%%%%
\begin{figure}[tb]
\begin{center}
\includegraphics[scale=.45]{figs/TwoLoopSpanningCuts.eps}
\end{center}
\vskip -.5cm
\caption{\small A spanning cuts that determine the full integrand other than quantum bubble
  on external leg contributions.  The complete set of cuts is given
  including all distinct labels and routing of different particles through the
  cuts. The lines represent on-shell particles of any type.
}
\label{TwoLoopSpanningCutsFigure}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 

In this section  we describe the construction of the two-loop gravity
integrand using both four-dimensional helicity and $D$-dimensional methods 
and show explicitly that the four-dimensional construction is sufficient to capture
all contributions to the classical potential in four space-time dimensions. 
%
As a warmup, we first analyze the simpler case of color-ordered gauge-theory 
four-scalar amplitude, pointing out various features of the construction that carry 
over to the gravity case.

As at one loop, we use the generalized unitarity
method~\cite{GeneralizedUnitarity}, briefly summarized in
\sect{IntegrandsSection}, to construct the two-loop integrand.  The complete
quantum integrand can be obtained using a spanning set of cuts,
which amounts to the set of cuts from which every term in the loop
integrand can be determined.  For the two loop massless case such a set is
shown in \fig{TwoLoopSpanningCutsFigure}, where all distinct
labeling and routings of different particles need to be
included. In the massive case there are additional contributions not captured by these cuts, related 
to bubbles on external legs, but these are purely quantum effects
which we ignore.

%%%%%%%%%%%%%% FIGURE %%%%%%%%%%%%%
\begin{figure}[tb]
\begin{center}
\includegraphics[scale=.5]{figs/TwoLoopCuts.eps}
\end{center}
\vskip -.5cm
\caption{\small The independent generalized cuts needed at two loops for the classical potential.
The remaininig contributing cuts are given by simple relabeling of external legs.  Here the straight
ines represent on-shell scalars and the wiggly lines correspond to on-shell gravitons or gluons.}
\label{TwoLoopCutsFigure}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 

%%%%%%%%%%%%%% FIGURE %%%%%%%%%%%%%
\begin{figure}[tb]
\begin{center}
\includegraphics[scale=.5]{figs/TwoLoopDiscardedCuts.eps}
\end{center}
\vskip -.5cm
\caption{\small Examples of cuts that are discarded because they have no
  further classical or iteration contributions to the potential that
  are not already found in the cuts of \fig{TwoLoopCutsFigure}.}
\label{TwoLoopDiscardedCutsFigure}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 


The set of cuts needed to determine the classical potential is, in fact,
a subset of the spanning set.  As explained in \sect{QuantumVsClassicalSection}, the only
unitarity cuts that can contain pieces of the classical potential
separate the two massive lines on opposite sides of the cut and have
one cut matter line in each loop.  In addition there are no
contributions from diagrams containing a graviton propagator starting and ending 
on the same scalar line.  
%
After dropping from the spanning set all unitarity cuts that do not contain any 
new contributions that satisfy these criteria, we are left with the cuts 
in \fig{TwoLoopCutsFigure}, together with independent ones obtained from relabeling 
the external lines.  
%
The first two cuts,  (a) and (b), are just the three-particle cut shown in \fig{TwoLoopSpanningCutsFigure}(a), 
where the three cut lines are gravitons, but with the additional requirement that one matter line per loop should
also be cut.  Similarly, the cut in
\fig{TwoLoopCutsFigure}(c) is just the iterated two-particle cut in \fig{TwoLoopSpanningCutsFigure}(b), 
with all cut lines being gravitons, but with the additional condition imposed that one matter line per
loop is cut.  Any other cuts, such as the ones shown in
\fig{TwoLoopDiscardedCutsFigure}, will contain pieces either already determined by
the cuts in \fig{TwoLoopCutsFigure}, or diagrams that do not contribute to the conservative potential.  
In particular, there are no new classical potential pieces in any iterated two particle cut of the form 
in \fig{TwoLoopSpanningCutsFigure}(c).

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Warmup: Gauge-Theory Generalized Cuts in Four Dimensions}

Before turning to gravity, we first evaluate the cuts in
\fig{TwoLoopCutsFigure} for a scalar-coupled gauge theory.  Once the
gauge-theory cuts have been determined, the gravity ones are obtained
easily through double copy.

As in the four-dimensional one loop construction, we take the amplitude to be color ordered
so we preserve the cyclic ordering of legs when writing out the tree amplitudes that compose the cut. 
The first two cuts in \fig{TwoLoopCutsFigure} are given by
\begin{align}
C_{\rm YM}^{\rm (a)} & = \!\sum_{h_5, h_6, h_7 = \pm} \!
A_3^\tree(3^s, -7^{-h_7}, -9^s) \, A_3^\tree(9^s, -6^{-h_6}, -8^s) \, 
\nonumber \\
&\hspace{3.5cm} \times A_3^\tree(8^s, -5^{-h_5}, 2^s)  A^\tree_5(1^s, 5^{h_5}, 6^{h_6}, 7^{h_7}, 4^s)  \,,
\label{WCutGT} \\
%
C_{\rm YM}^{\rm (b)} & =\! \sum_{h_5, h_6, h_7 = \pm} \!
A_4^\tree(3^s, -7^{-h_7}, -6^{-h_6},-8^s) \, A_3^\tree(8^s, -5^{-h_5}, 2^s) \nonumber \\
&\hspace{3.5cm} \times A^\tree_4(1^s, 5^{h_5}, 6^{h_6}, 9^{s})   \, A_3^\tree(-9^s, 7^{h_7}, 4^s) \,.
\label{NCutGT}
\end{align}
The helicity sums run over $2^3=8$ possible configurations:
\begin{equation}
\{ h_5, h_6, h_7 \} : \,
\{+++ \}, 
\{--- \},
\{+--\}, 
 \{-++\}, 
\{+-+\}, 
\{-+-\}, 
\{++-\}, 
\{--+\} \ .
\label{3CutHelicities}
\end{equation}
Similarly, the cut in \fig{TwoLoopCutsFigure}(c) is, 
%
\begin{align}
C_{\rm YM}^{\rm (c)} = \sum_{h_5, h_6, h_7, h_8 = \pm} \!
A^\tree_3(3^s, 7^{h_7}, -9^s) \, A^\tree_3(9^s,  -8^{-h_8}, 2^s) \,
 A^\tree_4(-5^{-h_5}, 8^{h_8},  -7^{-h_7},  6^{h_6}) \nn \\
\times A^\tree_3(1^s,5^{h_5}, -10^s) A^\tree_3(10^s, -6^{-h_6},4^s) \,,
\label{HCutGT}
\end{align}
where legs $ 5, 6, 7, 8$ are cut gluon lines and $9$ and
$10$ are cut matter lines.  The sum over helicity configurations runs 
over
\begin{equation}
\{ h_5, h_6, h_7, h_8 \} : \,
\{++++ \},  \; \{----\}, \; \{+--+\}, \; \{++--\}, \; \{--++\}, \; \{-++-\} \ .
\label{HCutHelicitiesGT}
\end{equation}
%corresponding to the helicity labels in \eqn{HCut}.  
The helicity labels correspond to the momentum flow indicated in \fig{TwoLoopCutsFigure}(c).  
All other configurations give vanishing contributions, because the four-gluon amplitude represented by the central blob vanishes
except for configurations with two legs of positive helicity and two of negative helicity for all outgoing momenta.  

As we encountered at one loop, each cut contains both terms that do not 
appear in any other cut  and terms that do. For example, the cut in \fig{TwoLoopCutsFigure}(a)
contains a term in which the lines 1, 4, 5, 6, 7 meet at a single five-point vertex which does not appear
in any other cut. It also contains a term corresponding to a two-loop planar double-box graph topology, 
which also appears in the cut in \fig{TwoLoopCutsFigure}(b).
% 
While we can simplify the cuts following a similar strategy as at one loop,
the process of organizing the result in terms of local diagrams and removing such double-counted terms
is more complex at two loops.
%
Instead, we will use the simple strategy where the cuts in Eqs.~\eqref{WCutGT}, \eqref{NCutGT} and~\eqref{HCutGT} are 
directly matched onto the cuts of an ansatz for the integrand with the desired local properties.  
In this way we simultaneously remove any overcount of terms in cuts and organize the result in terms of Feynman integrals.

To illustrate some important features and to explain the terms that can be
dropped when evaluating the cuts in four dimension, we will summarize the calculation of the cut in \fig{TwoLoopCutsFigure}(c).
In particular, we explain in \sect{sec:evanescence} ambiguities in the integrand when working in four dimensions  and why they 
do not affect the classical potential.

Following similar algebraic steps as at one loop and using standard spinor
manipulations we evaluate the terms in the cut in \fig{TwoLoopCutsFigure}(c) given by the different 
helicity configurations in \eqn{HCutGT}.  We find
\begin{align}
&C_{\rm YM}^{\{++++\}} = 
 - i \frac{m_1^2 m_2^2 \,t } {(- \t_{58}) } \,, 
%
&C_{\rm YM}^{\{+--+\}} =
   -i\frac{\tr^2_-[7 2 8 6 1 5] }
   {t^3  (- \t_{58}) } \, , \quad
%
&C_{\rm YM}^{\{+-+-\}} =
-i\frac{ \tr^2_-[8 2 7 6 1 5] }
{t^3 (- \t_{58})}\,,  \nn\\ 
%
&C_{\rm YM}^{\{----\}}  =
- i \frac{m_1^2 m_2^2 \, t } { (- \t_{58})} \,,
%\hskip 1.45 cm 
%
&C_{\rm YM}^{\{-++-\}} = 
  -i\frac{\tr^2_+7 2 8 6 1 5]}
  {t^3  (- \t_{58}) } \, ,\quad
%
&C_{\rm YM}^{\{-+-+\}}  =
-i\frac{ \tr^2_+[8 2 7 6 1 5] }
{t^3 (- \t_{58})} \, .
\label{YMHCutResult}
\end{align}

While not necessary for the construction of the color-ordered two-loop
scalar amplitude with the ordering ${\rm
  Tr}[T^{a_1}T^{a_2}T^{a_3}T^{a_4}]$, to construct the gravity cut
corresponding to \fig{TwoLoopCutsFigure}(c) using the KLT relations we
also need the twisted color-ordered cut, obtained by exchanging $\{-5
\leftrightarrow 6 \}$ in the four-point tree-amplitude factor,
\begin{align}
C_{\rm YM}^{\prime \rm (c)} = \sum_{h_5, h_6, h_7, h_8 = \pm} \!
A_3^\tree(2^s,  9^s,  -8^{-h_8}) \, A_3^\tree(7^{h_7},-9^s, 3^s) \, 
 A^\tree_4(6^{h_6}, 8^{h_8},  -7^{-h_7}, -5^{h_5}) \nn \\
\times A^\tree_3(1^s,5^{h_5}, -10^s) A^\tree_3(10^s, -6^{-h_6},4^s) \, .
\label{YMHCutPrimeResult}
\end{align}
The sum runs over the helicity configurations in \Eq{HCutHelicitiesGT}. Using the BCJ amplitudes relation in \eqn{eq:fund_BCJ},
\begin{equation}
A^\tree_4(6^{h_6}, 8^{h_8},  -7^{-h_7}, -5^{h_5}  ) = -\frac{\t_{58}}{\t_{68}} 
    A^\tree_4(-5^{h_5}, 8^{h_8}, -7^{-h_7}, 6^{h_6} ) \,,
\end{equation} 
it is not difficult to find that the twisted cut and its helicity-labeled components are simply
\begin{equation}
C_{\rm YM}^{\prime \{h_5, h_6, h_7, h_8\}}  =  \frac{(- \t_{58})} {\t_{68}} C_{\rm YM}^{\{h_5, h_6, h_7, h_8\}} \, ,
\hskip 1cm
C_{\rm YM}^{\prime \rm (c)}  =  \frac{(- \t_{58})} {\t_{68}} C_{\rm YM}^{\rm (c)} \, .
\label{FinalTwisted}
\end{equation}
The rational factor effectively replaces the $-1/\t_{58}$ propagator with the  $1/\t_{68}$ one, corresponding to the relabeled
four-point amplitude in the middle blob in \fig{TwoLoopCutsFigure}(c).


Next, we evaluate the two remaining traces in \Eq{YMHCutResult}. We split them into parity-even and
parity-odd parts, as at one-loop, resulting in
\begin{align}
\tr_\pm^2[8 2 7 6 1 5]  & =  {\cal E}_1^2 + {\cal O}_1^2 \pm 2 {\cal O}_1 {\cal E}_1\, ,
\label{TraceTwoLoop1}
\\
\tr_\pm^2[7 2 8 6 1 5]  & =  {\cal E}_2^2 + {\cal O}_2^2 \pm  2 {\cal O}_2 {\cal E}_2\, .
\label{TraceTwoLoop2}
\end{align}
It is however clear that, in the complete cut, the parity-odd part cancels out, so we only need to compute ${\cal O}_i^2$.
%
Evaluating the trace using standard gamma-matrix identities we find  
\begin{align}
{\cal E}_1^2 & = 
\frac{1}{4}  t^2 \bigl(\t_{1 2} \t_{5 8} - \t_{1 8}\t_{2 5} \bigr)^2 \,,
\qquad
{\cal O}_1^2 = {\cal E}_1^2 - \t_{5 8}^2 m_1^2  m_2^2 \, t^2  \,.
\label{EvenOddOne}
\\
{\cal E}_2^2 & = 
\frac{1}{4} t^2 \bigl( \t_{24} \t_{5 7} + \t_{1 7} \t_{57} \bigr)^2 \,,
\qquad
{\cal O}_2^2 = {\cal E}_2^2 - \t_{5 7}^2 m_1^2 m_2^2 \, t^2 \,,
\label{EvenOddTwo}
\end{align}
where $t = (p_2 + p_3)^2$ and $\t_{i j} = 2 p_i \cdot \ell_j$.

Adding up the contributions of the six helicity configurations, we find that the complete 
four-dimensional cut in \fig{TwoLoopCutsFigure}(c) is given by
\begin{align}
\label{full4dHcutGT}
C_{\rm YM}^{\rm (c)}
& = -2  i \frac{1} {(-\t_{58})}
   \biggl[m_1^2 m_2^2 t + \frac{1}{t^3} \bigl(
 {\cal E}_1^2 + {\cal O}_1^2  +  {\cal E}_2^2 + {\cal O}_2^2 \bigr) \biggr] \\
%
& = -2  i \frac{1} {(-\t_{58})}
   \biggl[m_1^2 m_2^2 t + \frac{1}{2 t} \bigl(
     (\t_{1 2} \t_{5 8} - \t_{1 8}\t_{2 5})^2 - 2 \t_{5 8}^2 m_1^2  m_2^2 + 
     (\t_{24} \t_{5 7} + \t_{1 7} \t_{57})^2 - 2 \t_{5 7}^2 m_1^2 m_2^2 \bigr) \biggr] \, .
     \nn
\end{align}
The twisted cut is simply obtained through \eqn{FinalTwisted}.


If naively continued outside of four dimensions, the expression
\eqref{full4dHcutGT} contains a spurious singularity.  To expose this
issue we construct the maximal cut obtained by imposing the additional
cut condition
\begin{equation}
\t_{5 8} = 0 \,.
\end{equation}
Together with the initial six cut conditions, this corresponds to
cutting the maximum number of propagators for a four-point two-loop
amplitude; consequently, the result should be local, as can be checked
by solving the seven cut conditions in four dimensions. However, with
this additional cut condition, we get the maximal cut interpreted as a
$D$-dimensional expression
\begin{equation}
C_{\rm YM}^{\rm max cut}  = -  \frac{1}{ t} \,\t_{1 8}^2 \, \t_{2 5}^2 \, .
\end{equation}
It contains a $1/t$ pole.  Maximal cuts should be local, since they are nothing more than 
sums of products of three vertices. This strongly suggests that the correct $D$ dimensional expression 
is missing a term proportional to a Gram determinant that vanishes in four
dimensions but not in $D$ dimensions.

This is indeed the case. To remove the spurious $1/t$ singularity we add a term proportional to the Gram determinant
 \begin{equation}
G_5  = 16 \det
\left( \begin{matrix}
  p_1  \cdot p_1 &  p_1  \cdot p_2 &  p_1 \cdot p_3 &   p_1\cdot \ell_5 &   p_1\cdot \ell_8 \\
  p_2  \cdot p_1 &  p_2  \cdot p_2 &  p_2 \cdot p_3 &   p_2\cdot \ell_5 &   p_2\cdot \ell_8 \\
  p_3  \cdot p_1 &  p_3  \cdot p_2 &  p_3 \cdot p_3 &   p_3\cdot \ell_5 &   p_3\cdot \ell_8 \\
  \ell_5  \cdot p_1 &  \ell_5  \cdot p_2 &  \ell_5 \cdot p_3 &   \ell_5\cdot \ell_5 &   \ell_5\cdot \ell_8 \\
  \ell_8  \cdot p_1 &  \ell_8  \cdot p_2 &  \ell_8 \cdot p_3 &   \ell_8 \cdot \ell_5 &   \ell_8\cdot \ell_8 
\end{matrix} \right),
\label{GramDete}
\end{equation}
which vanishes in four dimensions.  By adjusting the coefficient of $G_5$ we can 
remove the spurious singularity.  This results in a cut that is now valid in $D$-dimensions,
\begin{align}
\label{improvedcutcGT}
C_{\rm YM} = -2  i \frac{1} {(-\t_{58}) }
   \biggl[ m_1^2 m_2^2 t + \frac{1}{t^3} \Bigl({\cal E}_1^2 + {\cal O}_1^2  +  {\cal E}_2^2 + {\cal O}_2^2  - t\,  G_5 \Bigr)\biggr] \,,
\end{align}
where the state-counting parameter is $D_s =4$. 
An alternative way to arrive at the same result is to match an ansatz written in terms of local 
diagrams (which by definition have no spurious singularities) onto $C_\text{YM}^{(c)}$.
%
The twisted cut can be obtained from  \eqn{improvedcutcGT} via \eqn{FinalTwisted}.


\subsection{Gravity Generalized Cuts in Four Dimensions}

The KLT relations~\eqref{KLT} provide a simple path for assembling the gauge-theory 
cut components constructed above into analytic expression for the three gravity cuts in \fig{TwoLoopCutsFigure}.
Those corresponding to \fig{TwoLoopCutsFigure}(a,b) are
\begin{align}
C_{\rm GR}^{\rm (a)} & = \sum_{h_5, h_6, h_7 = \pm} \!
M_3^\tree(2^s, 8^s, -5^{-h_5}) \, M_3^\tree(-6^{-h_6},-8^s, 9^s) \nn\\
& \hskip 3 cm \null \times
  M_3^\tree(7^{h_7},-9^s, 3^s) \, M_5^\tree(1^s, 5^{h_5}, 6^{h_6}, 7^{h_7}, 4^s) \,, 
\label{WCutGR} \\
%
C_{\rm GR}^{\rm (b)} & = \sum_{h_5, h_6, h_7 = \pm} \!
M_3^\tree(2^s, 8^s, -5^{-h_5}) \, M_4^\tree(-7^{-h_7}, -6^{-h_6},-8^s, 3^s) \nn \\
& \hskip 3 cm \null \times
 M^\tree_4(1^s, 5^{h_5}, 6^{h_6}, 9^s) \, M_3^\tree(-9^s, 7^{h_7}, 4^s)  \,,
\label{NCutGR}
\end{align}
where the helicity configurations run over the eight possibilities in \eqn{3CutHelicities}, except that here 
the $\pm$ refer to the spin states of gravitons instead of those of gluons.  The gravity tree amplitudes
can be simply evaluated using the KLT relations~\eqref{KLT}.
Similarly, the remaining cut in~\fig{TwoLoopCutsFigure}(c) is 
%
\begin{align}
C_{\rm GR}^{\rm (c)} & = \sum_{h_5, h_6, h_7, h_8 = \pm} \!
M^\tree_3(2^s,  9^s,  -8^{-h_8}) \, M^\tree_3(7^{h_7},-9^s, 3^s) \, 
 M^\tree_4(-5^{-h_5}, 6^{h_6}, -7^{-h_7}, 8^{h_8} ) \nn \\
& \null \hskip 4 cm 
\times M^\tree_3(1^s,5^{h_5}, -10^s) M^\tree_3(10^s, -6^{-h_6},4^s) \nn \\
%
& = -i t
\sum_{h_5, h_6, h_7, h_8 = \pm} 
\biggl[ A^\tree_3(2^s,  9^s,  -8^{-h_8}) \, A^\tree_3(7^{h_7},-9^s, 3^s) \, 
 A^\tree_4(-5^{-h_5}, 6^{h_6}, -7^{-h_7}, 8^{h_8} ) \nn \\
& \null \hskip 4 cm 
\times A^\tree_3(1^s,5^{h_5}, -10^s) \, A^\tree_3(10^s, -6^{-h_6},4^s) \biggr] \nn\\
& \hskip 2.75 cm \null \times
\biggl[ A^\tree_3(2^s,  9^s,  -8^{-h_8}) \, A^\tree_3(7^{h_7},-9^s, 3^s) \, 
 A^\tree_4(6^{h_6}, 8^{h_8},  -7^{-h_7}, -5^{h_5} ) \nn \\
& \null \hskip 4 cm 
\times A^\tree_3(1^s,5^{h_5}, -10^s) \, A^\tree_3(10^s, -6^{-h_6},4^s) \biggr]
\,,
\label{HCutGR}
\end{align}
where legs $ 5, 6, 7, 8$ are cut graviton lines and $9$ and $10$ are cut matter lines.  
As for the gluon case, some helicity configurations have vanishing contributions because of the properties 
of the four-graviton amplitude factor, 
so the  sum over helicities  in \eqn{HCutGR} effectively runs over the configurations in \eqn{HCutHelicitiesGT}.
%
As at one loop, we project out the dilaton and axion simply by requiring that the helicities of gluons in the two 
gauge-theory factors  in Eqs.~\eqref{WCutGR}, \eqref{NCutGR} and \eqref{HCutGR}   be identical.


Upon using the gauge-theory tree amplitudes given in \app{TreeAmplitudesAppendix} we find compact expressions
for the three types of cuts in \fig{TwoLoopCutsFigure}, which can subsequently be assembled into a single integrand, as we discuss below.
%
It is instructive to inspect in some detail the cut in \fig{TwoLoopCutsFigure}(c),  in order to understand potential issues with 
carrying out the calculation in four dimensions compared to $D$ dimensions.  In general, we prefer the four-dimensional 
expressions because their complexity at higher loops increases slower than that of their $D$-dimensional counterparts.

The cut components, labeled by the helicities of the cut graviton lines in \fig{TwoLoopCutsFigure}(c) 
are obtained through the KLT relations in terms of the direct and twisted YM cut components 
in \eqns{YMHCutResult}{YMHCutPrimeResult}
\begin{align}
C_{\rm GR}^{\{h_1 h_2 h_3 h_4\}} 
&  = -i \, t \, C_{\rm YM}^{\{h_1 h_2 h_3 h_4\}} C_{\rm YM}^{\prime \{h_1 h_2 h_3 h_4\}} \, .
\end{align}
As explained above, by identifying the helicity labels in the two gauge-theory amplitudes we project out the dilaton and axion 
contributions to cuts. 
%
Using the relation in \eqn{FinalTwisted}, we can read off the results in different helicity configurations as
\begin{align}
&C_{\rm GR}^{\{++++\}}   = 
 i \frac{m_1^4 m_2^4 t^3 } { (-\t_{58})  \t_{68}} \,,
%
&C_{\rm GR}^{\{+--+\}}   =
 i\frac{\tr^4_-[7 2 8 6 1 5] }
{t^5  (-\t_{58}) \t_{68}} \,, \quad\;
%
&C_{\rm GR}^{\{+-+-\}}   =
i\frac{ \tr^4_-[8 2 7 6 1 5] }
{t^5 (-\t_{58}) \t_{68}} \,, \nn \\ 
%
&C_{\rm GR}^{\{----\}}   =
 i \frac{m_1^4 m_2^4 t^3 } { (-\t_{58})  \t_{68}} \,,
%
&C_{\rm GR}^{\{-++-\}}   = 
i\frac{\tr^4_+[7 2 8 6 1 5]}
{t^5  (-\t_{58})  \t_{68}} \,, \quad\;
%
&C_{\rm GR}^{\{-+-+\}}   =
   i\frac{ \tr^4_+[8 2 7 6 1 5] }
   {t^5 (-\t_{58}) \t_{68}} \,.
\label{GRHCutResult}
\end{align}
Summing over all helicity configurations of gravitons crossing the iterated two-particle cuts, we find
\begin{align}
C_{\rm GR}^{\rm (c)} & = 
 -i \biggl[ 2 t^2 m_1^4 m_2^4 + \frac{1}{t^6} \Bigl(
  \tr^4_-[7 2 8 6 1 5] +
  \tr^4_-[8 2 7 6 1 5] +
  \tr^4_+[7 2 8 6 1 5] +
  \tr^4_+[8 2 7 6 1 5] \Bigr)
\biggr] 
%\nn \\
%&\hskip 2 cm \null \times
%
 \biggl[\frac{1}{(-\t_{58})} + \frac{1}{\t_{68}}
          \biggl] \,,
\label{GRcutC}          
\end{align}
where we used the partial fractioning identity (recall that momenta are flowing as indicated in~\fig{TwoLoopCutsFigure}(c))
\begin{align}
\frac{1}{ (-\t_{58}) \t_{68}}
 & = - \frac{1}{t} \biggl[\frac{1}{(-\t_{58})} + \frac{1}{\t_{68}}
          \biggl]\, .
\end{align}
%As always because we control the helicities that cross the cut there is no
%contamination from dilatons or axions. 
By inspecting \eqn{GRcutC} it is easy to see that all parity-odd terms cancel out.
%
We can evaluate the traces using \eqns{TraceTwoLoop1}{TraceTwoLoop2}
\begin{align}
\label{GCfullC}
C_{\rm GR}^{\rm (c)} & =
  -2i \biggl[  t^2 m_1^4 m_2^4 + \frac{1}{t^6} \Bigl(
  {\cal E}_1^4 + {\cal O}_1^4 + 6 {\cal O}_1^2 {\cal E}_1^2 +
  {\cal E}_2^4 + {\cal O}_2^4 + 6 {\cal O}_2^2 {\cal E}_2^2  \Bigr)
\biggr]
 \biggl[\frac{1}{(-\t_{58})} + \frac{1}{\t_{68}}
          \biggl] \,,
\end{align}
where the even-squared and odd-squared terms are given in
Eqs.~~\eqref{EvenOddOne} and  \eqref{EvenOddTwo}.

As for the YM cut with the same topology, if we naively extend \eqn{GCfullC} to $D$ dimensions we encounter 
a spurious singularity in the maximal cut, which we can remove by adding in \eqn{GramDete} a term proportional to the Gram determinant, 
that vanishes in four dimensions.  Doing so gives,
\begin{align}
C_{\rm GR}^{\rm (c)} & =
  -2i \biggl[  t^2 m_1^4 m_2^4 + \frac{1}{t^6} \Bigl(
  {\cal E}_1^4 + {\cal O}_1^4 + 6 {\cal O}_1^2 {\cal E}_1^2 +
  {\cal E}_2^4 + {\cal O}_2^4 + 6 {\cal O}_2^2 {\cal E}_2^2
% \nn \\
% & \hskip 4 cm \null
   -2 t G_5  ( {\cal E}_1^2 + {\cal O}_1^2  +  {\cal E}_2^2 + {\cal O}_2^2) 
   + t^2 G_5^2\Bigr) \biggr] \nn \\
& \hskip 2cm  \times 
 \biggl[\frac{1}{(-\t_{58})} + \frac{1}{\t_{68}}
          \biggl] \,.
          \label{GCfullCnaiveDextension}
\end{align}
As we will see, further terms that vanish in four dimensions (and therefore proportional to $G_5$) are necessary to 
obtain the complete $D$-dimensional cut. 
Nevertheless, all terms proportional to $G_5$ do not contribute to the classical  potential, as we discuss in \sect{sec:evanescence}.

For comparison, the cut in \fig{TwoLoopCutsFigure}(c) for the scattering of scalars coupled to a graviton, dilaton and antisymmetric tensor
(or axion) is given by the simple double copy:
\begin{align}
C_{\rm GR}^{\rm (c)} +  C_{\rm \phi a}^{\rm (c)} & =
  -4i \biggl[  t m_1^2 m_2^2 + \frac{1}{t^3} \Bigl(
  {\cal E}_1^2 + {\cal O}_1^2  + {\cal E}_2^2 + {\cal O}_2^2  - t G_5  \Bigr) \biggr]^2
 \biggl[\frac{1}{(-\t_{58})} + \frac{1}{\t_{68}} \biggl]\, .
\end{align}
This expression holds for kinematics in general dimension, but with $D_s = 4$.

%%%%%%%%%%%%%

\subsection{$D$-Dimensional Generalized Cuts}

The evaluation of the $D$-dimensional version of the generalized cuts in \fig{TwoLoopCutsFigure} 
is similar to the evaluation of the one-loop $D$-dimensional cuts in \sect{OneLoopSection}, except that the relevant gauge-theory 
trees are somewhat more complicated.  Besides the two-scalar three-gluon tree-level amplitude needed for the cut in
\fig{TwoLoopCutsFigure}(a), we also need the four-gluon amplitude in a
BCJ form that also satisfies the on-shell Ward identity \eqn{GeneralizedWardIdentity} without use of transversality of 
the external states.  
%
These tree amplitudes are given in \app{TreeAmplitudesAppendix}.  
By using a good basis choice and BCJ duality, the amplitudes are determined by specifying a single
numerator.  Because BCJ duality is manifest, the desired gravity cuts follow immediately from the gauge-theory ones through
the double-copy substitution in \Eq{ColorSubstitution}.

As at one-loop, we exploit the compact physical-state projector in \eqn{SimplifiedGravitonProjector}, which is a consequence of
the on-shell Ward identities holding without imposing the transversality of gluon and graviton asymptotic states and of the decoupling of antisymmetric tensor.
This trick simplifies the two-loop calculation enormously.
We will not include the details since the calculations are straightforward extensions of the one-loop ones. 
%
We will however comment on the result for the cut in \fig{TwoLoopCutsFigure}(c) and compare it with the four-dimensional
expression in \Eq{GCfullC}.

Taking $D_s = \eta_\mu^{\ \mu} = 4$, the cut in \fig{TwoLoopCutsFigure}(c) evaluates to the rather compact expression
\begin{align}
C_{\rm GR}^{\rm (c)}  =&
  -2i \biggl[  t^2 m_1^4 m_2^4 + 
  \frac{1}{t^6} \Bigl(
  {\cal E}_1^4 + {\cal O}_1^4 + 6 {\cal O}_1^2 {\cal E}_1^2 +
  {\cal E}_2^4 + {\cal O}_2^4 + 6 {\cal O}_2^2 {\cal E}_2^2 %\nn \\
%& \hskip 4 cm \null
   -2 t G_5  ( {\cal E}_1^2 + {\cal O}_1^2  +  {\cal E}_2^2 + {\cal O}_2^2)
   + t^2 G_5^2 \Bigr) \nn \\
& \qquad
   - \frac{1}{t}  ( 2 m_1^2 m_2^2 + (\t_{1 2} - \t_{1 8} + \t_{2 5} - \t_{5 8})^2 ) G_5
 \biggr]  \biggl(\frac{1}{(-\t_{58})} + \frac{1}{\t_{68}} \biggl) \ ,
\end{align}
where $G_5$ is the Gram determinant in \eqn{GramDete}.  We note that,
apart from the $G_5$ terms we found by requiring absence of a spurious
pole in the maximal cut of the naive $D$-dimensional continuation of
the four-dimensional result in \Eq{GCfullCnaiveDextension}, the
complete $D$-dimensional calculation yields additional terms linear in
$G_5$.
%
The other cuts are also straightforward to evaluate, although we have not obtained compact $D$-dimensional expressions for them.

%%%%%%%%%%%%%%%%%
\subsection{Merging the Cuts into an Integrand}
\label{MergingSubsection}

%%%%%%%%%%%%%% FIGURE %%%%%%%%%%%%%                                                                    
\begin{figure}
\begin{center}
\includegraphics[scale=.5]{figs/MasterDiags.eps}
\end{center}
\vskip -.5cm
\caption{\small The eight independent diagrams with only cubic vertices
  showing the propagator structure of integrals which contribute to
  the classical potential. The thick lines correspond to massive
  particles.  All other diagrams are given by relabeling the external legs. In the main text, we will denote each diagram using bold label, e.g. diagram $\bm 1$ for the first diagram.
  }
\label{MasterDiagsFigure}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%                                                                   


Once the cuts have been evaluated, the next step is to reorganize them into an integrand.  
We do this for both their four and $D$-dimensional versions. 
While obtaining the integrand from the four-dimensional cuts turns out to be sufficient, it is nevertheless important 
to verify that no subtleties arise from truncating the integrand to four-dimensions, given the fact that the
integrated amplitude is infrared divergent.

In general, different unitarity cuts contain information about the same terms in the integrand.  
For example, contributions to diagram $\bm 1$ in \fig{MasterDiagsFigure} are found in both cuts (a) 
and (b) of \fig{TwoLoopCutsFigure} while contributions to diagram $\bm 7$ in \fig{MasterDiagsFigure} 
appear both in cuts (b) and (c) of \fig{TwoLoopCutsFigure}.  
%
Such double counting can be removed either during the construction of
the integrand ~\cite{BDDPR,TwoLoopSplitting} or after
integration~\cite{Bern:2002tk}. We will choose the former approach, as
it meshes well with our integration methods described in the next
sections.

To determine the numerators for the diagrams in
\fig{MasterDiagsFigure} we construct an ansatz for each of them. While
contact diagrams with four- or higher-point vertices can be included
in the ansatz, we choose to minimize the number of independent graphs
by instead using diagrams that have only cubic vertices as shown in
\fig{MasterDiagsFigure}, and capturing contact terms by multiplying
and dividing by appropriate propagators.
%
The highest number of loop-momentum factors in each term of the ansatz
follows from the two-derivative nature of gravity couplings, counting
two such factors for each three-point vertex. As we will see, it is
not necessary to saturate the maximal power counting for all diagrams.
%
After including relabelings of external lines, the eight diagram
topologies shown in \fig{MasterDiagsFigure} are the minimal set needed
for matching the three unitarity cuts in~\fig{TwoLoopCutsFigure}.
%
We imposing the natural requirement that the symmetries of a diagram
are also symmetries of its numerator factor.  The parameters of the
ansatze are then fixed by computing their generalized cuts (including
contributions from the relabelings) and match to those
in~\fig{TwoLoopCutsFigure} computed earlier via multiplying tree
amplitudes.  Once this is done, the merged integrand simultaneously
satisfies all other generalized unitarity cuts related to
\fig{TwoLoopCutsFigure} by exchanging the external legs, because the
relabeling is built-in explicitly.

 
An observation that leads to simplifications when imposing diagram
symmetries is that on-shell conditions may be imposed on a given leg
in a given diagram if that leg is on-shell in {\em all} cuts that
contribute to that diagram.
%
For example, the on-shell conditions for the three gravitons can be
applied to the numerator of diagram $\bm 1$ because these gravitons
are on shell in both cuts (a) and (b) in \fig{TwoLoopCutsFigure}.  The
four gravitions that connect to matter lines in diagram $\bm 7$ must
however be treated off shell because they are off shell in cut (b) in
\fig{TwoLoopCutsFigure}.
%
On the other hand, we can use the on shell condition for the two
matter lines in diagrams $\bm 7$ and $\bm 8$ without affecting the
classical potential because only cuts (b) and (c) in
\fig{TwoLoopCutsFigure} source them and they both place the matter
lines on shell.

In the construction of the ansatz for each diagram's numerator, we only require a 
sufficiently high power of loop momenta
such that a solution exists and matches either to four-dimensional cuts
or to $D$ dimensional cuts.  
%
For example, diagram $\bm 1$ in \fig{MasterDiagsFigure} does not require
any powers of loop momenta in the numerators, while the numerator of
diagram $\bm 6$ requires the maximum of 12 powers of loop momenta to
match the cuts, prior to dropping quantum terms containing more than 4
powers of loop momenta in the numerator.  

In general, the numerators contain free parameters because of the possibility of
assigning the same contact term to different diagrams without changing
the value of integrand.
We choose the remaining undetermined parameters to simplify the matching with the effective field 
theory amplitudes in \sect{sec:EFT}. For example, we chose diagram (1) to have a numerator proportional to the third power 
of the numerator in tree-level four-scalar amplitude, i.e.
\begin{equation}
N^{(1)}_{\rm GR}(1,2,3,4) =  \left((s - m_1^2 - m_2^2)^2 -\frac{4}{D_s-2} m_1^2 m_2^2 \right)^3 \,.
\end{equation}
By imposing diagram's symmetry on all numerators, simple relabeling gives us the value of the numerators 
with swapped legs.  For example,  the numerator corresponding to the case where legs 1 and 4 are swapped 
is simply,
\begin{equation}
N^{(1)}_{\rm GR}(1,3,2,4) =  \left((u - m_1^2 - m_2^2)^2 -\frac{4}{D_s-2} m_1^2 m_2^2 \right)^3 \,.
\end{equation}
The numerators of the other diagrams are more involved. The free parameters also provide a nontrivial check 
since they should cancel out in the final integrated amplitude. We have performed extensive checks to confirm this property. 

% % 
\begin{table}[t]
	\centering 
	\def\arraystretch{1.2}
	\begin{tabular*}{0.7 \textwidth}{c  @{\extracolsep{\fill}} l}
		\hline\hline
		Graph & External relabeling \\
		\hline
		1 & (1 2 3 4),\, (1 3 2 4)\\
		2 & (1 2 3 4),\, (1 3 2 4),\, (4 3 2 1),\, (4 2 3 1),\, $+\{1,4\} \leftrightarrow \{2,3\}$\\
		3 & (1 2 3 4),\, (1 3 2 4),\, $+\{1,4\} \leftrightarrow \{2,3\}$\\
		4 & (1 2 3 4),\, (1 3 2 4),\, (4 3 2 1),\, (4 2 3 1)\\
		5 & (1 2 3 4),\, (4 2 3 1),\, $+\{1,4\} \leftrightarrow \{2,3\}$\\
		6 & (1 2 3 4),\, $+\{1,4\} \leftrightarrow \{2,3\}$\\
		7 & (1 2 3 4),\, (1 3 2 4) \\
		8 & (1 2 3 4) \\
		\hline \hline
	\end{tabular*}
	\caption{\small List of 27 cubic diagrams from relabeling of the eight graphs in \fig{MasterDiagsFigure}. The right column gives all independent labels by exchanging the original external legs $(1 2 3 4)$ in each graph in \fig{MasterDiagsFigure}. Here $\{1,4\} \leftrightarrow \{2,3\}$ means swapping $1,4$ with $2,3$ in all the previous labels. For example, this yields (2 1 4 3) and (2 4 1 3) for graph 5.  }
	\label{table:assembly}
\end{table}
% % %

Once a valid set of numerators with the properties described above has been 
determined, we can treat the diagrams as if they were ordinary off-shell Feynman diagrams.  
In particular, the  diagram numerators are functions of the external labels and can 
be taken as respecting diagram symmetry. While on-shell conditions have been 
used in their construction, we can view their use as merely affecting terms with no 
contributions to the classical potential.

We write the part of the two-loop four-scalar amplitude necessary for
the extraction of the complete 3PM conservative potential as a sum
over 27 diagrams,
\begin{equation}
  M^{\rm 2\hbox{-}loop} = (4E_1 E_2)\,i\mathcal{M}_3 =  i (8 \pi G)^3 \int \frac{d ^D \ell_5}{(2 \pi)^D} \frac{d ^D\ell_6}{(2 \pi)^D}
           \sum_{i=1}^{27} {\cal I}^{(i)} \, ,
\end{equation}
%where we have use the standard relativistic normalization for scattering amplitudes. \draftnote{I would omit last clause}
where $\mathcal{M}_3$ is the 3PM amplitude including a nonrelativistic normalization $1/4E_1 E_2$. We will use this normalization for the amplitudes $\mathcal{M}_n$ presented in \sect{sec:scattering} and \sect{sec:EFT}.
The sum runs over 27 distinct diagrams arising from the independent relabelings of the external legs of the eight diagrams in~\fig{MasterDiagsFigure}, which are taken to correspond to $i=1,\dots,8$ and are found in the ancillary Mathematica text file {\tt masternumers.m}~\cite{AttachedFile}.  
The relabelings are listed in Table~\ref{table:assembly}.
The integrands are expressed 
in terms of numerators and denominators, in the usual way:
\begin{equation}
{\cal I}^{{i}} = \frac{N^{(i)}}{D^{(i)}} \, .
\end{equation}
The denominators are simply the Feynman propagators of the corresponding diagram.  
%
For example, for diagram (1) of 
\fig{MasterDiagsFigure},
\begin{equation}
D^{(1)} =  \ell_5^2 \ell_6^2  (\ell_5 +\ell_6 -p_2 - p_3)^2  (\ell_5 -p_2)^2  (\ell_5+ \ell_6 - p_2) ^2  (\ell_5 +p_1)^2  (\ell_5 +  \ell_6 + p_1)^2 \ ,
\end{equation}
where we have suppressed the standard Feynman $i\eps$ prescription,
which should be included for each propagator.  The numerators in this
file are valid in $D$ dimensions, but with the state-counting
parameter $D_s = 4$ for simplicity.

We have also constructed  several alternative integrands starting both from cuts constructed in four and $D$ 
dimensions, as described above. As already noted, expressions obtained with these two starting points differ
by terms proportional
to the Gram determinant $G_5$ in \Eq{GramDete}, which vanishes in four dimensions. In addition, when we use helicity methods, the state-counting parameter is automatically taken to be $D_s = 4$. We have explicitly checked
that integrands extracted from four dimensions and $D$ dimensions and
using $D_s=4$ or $D_s = 4 - 2 \eps$ lead to identical final results
for the potential.

The independence of the potential on the details of the dimensional
regularization prescription is not accidental.  In
\sect{sec:evanescence}, we explain why any two-loop integral
containing a Gram determinant that vanishes in four dimensions cannot contribute to the
classical potential and why the results are independent of the choice
of prescription for the $D_s$ parameter.  The net effect is that, 
analogous to the way as it works at one loop, the difference between
constructing the integrand in four and in $D$ dimensions does not affect the classical potential.  This, of course, agrees with naive expectations.


